RobustFill: Neural Program Learning under Noisy I/O

The problem of automatically generating a computer program from some specification has been studied since the early days of AI. Recently, two competing approaches for automatic program learning have received significant attention: (1) neural program synthesis, where a neural network is conditioned on input/output (I/O) examples and learns to generate a program, and (2) neural program induction, where a neural network generates new outputs directly using a latent program representation. Here, for the first time, we directly compare both approaches on a large-scale, real-world learning task. We additionally contrast to rule-based program synthesis, which uses hand-crafted semantics to guide the program generation. Our neural models use a modified attention RNN to allow encoding of variable-sized sets of I/O pairs. Our best synthesis model achieves 92% accuracy on a real-world test set, compared to the 34% accuracy of the previous best neural synthesis approach. The synthesis model also outperforms a comparable induction model on this task, but we more importantly demonstrate that the strength of each approach is highly dependent on the evaluation metric and end-user application. Finally, we show that we can train our neural models to remain very robust to the type of noise expected in real-world data (e.g., typos), while a highly-engineered rule-based system fails entirely.

==> dsl.tex <==
\section{Domain-specific Language}

\renewcommand{\t}[1]{\texttt{#1}}

\begin{figure}
\begin{center}
\begin{eqnarray*}
\mbox{String } e & := & \t{Concat}(f,e) \; | \; \t{A}(f) \; | \; f \nonumber \\
\mbox{Substring } f & := & \t{ConstStr}(s) \\
& | & \t{GetSpan}(r_1,k_1,d_1,r_2,k_2,d_2) \nonumber \\
& | & \t{SubStr}(k_1,k_2) \nonumber \\
\mbox{Direction } d & := & \t{Start} \; | \; \t{End} \nonumber \\
\mbox{Regex } r & := & T_1 \; | \; \cdots \; | \; T_n \; | \; \delta_1 \; | \; \cdots \; | \; \delta_m \nonumber \\
\mbox{API } \t{A} & := & \t{Get}(T,k) \; | \; \t{ToCase}(c) \; | \; \t{GetTo}(r,k) \nonumber \\
& | & \t{GetFrom}(r,k) \; | \; \t{Replace}(\delta_1,\delta_2)
\end{eqnarray*}
\end{center}
\caption{The Domain-specific language of regular expression based string transformations.}
\end{figure}

==> notes.tex <==
% I don't think this belongs in the modeling section

% \textit{Input Program}:

% {\tt ToCase(Lower, SubString(10, 15)) $|$ ConstStr(@)}

% \textit{Embedding Token Representation}:

% {\tt ToCase Case=Lower SubString k=10 k=15 \textbar\ ConstStr-@ \textbar\ </s>}

% The function nesting is unambiguous because all functions take a fixed number of parameters. The DSL semantics are not known to the neural decoder itself, but if it produces a program sequence which is invalid with respect to the DSL, the program executor will simply consider this a standard failure.\footnote{The decoder is unlikely to produce invalid programs since it was only trained on valid programs.} Also note that the numeric parameter values are represented as embeddings.\footnote{This does imply that the model cannot generalize to lengths beyond what it was trained on, but synthetic data can be generated up to any length. Our experiments use a max length of 100 characters for IO examples.}




% \subsection{Improving Beam Search}
% \label{sec:beam_search}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=225px]{images/beam_search_results.png}
% \caption{The generalization accuracy using for four search algorithm variants during decoding. Results were obtained using Attention-C.}
% \label{fig:beam_search_results}
% \end{figure}

% Because the goal of program synthesis is to generate a set of candidate programs, rather than to find the highest scoring 1-best output, it is reasonable to believe that standard beam search is can be improved upon for this task.

% Here, we consider four simple algorithms for decoding with a beam size $k$:
% \begin{enumerate}
% \item {\bf Monte Carlo}: There are $k$ independent decodes performed for each test instance (in parallel), where the next token is chosen with probability proportional to the output softmax distribution. 
% \item {\bf Beam}: The standard beam search used in most sequence generation tasks. At each timestep, each partial candidate is extended with all possible program tokens. These new hypotheses are sorted together by model score, and the top $k$ are kept.
% \item {\bf DP-Beam}: A variant of beam search which uses the dynamic programming-based candidate pruning described in Section~\ref{sec:search_space}. Every time an expression is completed in a given hypothesis (i.e., the ``{\tt \textbar}'' token is emitted), this partial program is evaluated in a black-box manner using the DSL. If the resulting string does not match a prefix of the observed {\tt OutStr}, the hypothesis is discarded.
% \item {\bf Diverse-DP-Beam}: The beam will often be filled with very similar candidates, especially with regard to emitting slightly different parameter tokens for the same set of functions. Here, we implement a simple heuristic to encourage function diversity: No single function sequence (excluding parameter tokens) can account for more than 20\% of the beam candidates. Many other methods for encouraging diversity could be explored in the future.
% \end{enumerate}

% Note that for a given beam size, the cost of all algorithms is effectively equal, since the total number of network evaluations is exactly the same. The beam search methods can produce more than $k$ candidates, but only the top $k$ candidates are considered for fairness of evaluation.

% Results are shown in Figure~\ref{fig:beam_search_results}. At a beam size of 100, standard beam search achieves 83\% accuracy, while DP-Beam achieves 88\% and Diverse-DP-Beam achieves 90\%. Monte Carlo search is significantly worse than all other approaches, especially for small beam sizes. The accuracy of 92\% with Attention-C + Diverse-DP-Beam=1000 is the strongest result reported in this paper. We do note that the DP-Beam variant is specific to concatenative DSLs, and may not be extendable to highly nested DSLs.




% The main differences between this work and \citet{parisotto2017} are:
% \begin{enumerate}
% \item {\bf Expressiveness of the DSL}: The DSL in \citet{parisotto2017} is missing the powerful ${\tt GetSpan}$ function, which is require for roughly 20\% of the FlashfillTest instances. Of course, this expressive power is not free -- this function alone increases the search space of the DSL by 10x, as discussed in Section~\ref{sec:search_space}. 
% \item {\bf Multi-example pooling}: \citet{parisotto2017} pools the final hidden states of the IO encoders, and only uses a single program decoder, whereas we use one decoder layer per IO example and pool their hidden state. However, we cannot draw direct conclusions about this since ``early pooling'' was not evaluated here.
% \item {\bf Attentional models}: Although \citet{parisotto2017} strongly model the relationship between the {\tt InStr} and {\tt OutStr} using cross-correlation, they do not strongly model the relationship between the program decoder and the IO. We have found that attentional models are critical for achieving high performance on this task.
% \item {\bf More accurate search}: \citet{parisotto2017} uses simple Monte Carlo sampling, which we demonstrate to be less accurate than standard beam search. Additional refinements to beam search improve our accuracy even further.
% \end{enumerate}





% \subsection{Approach}
% % todo: this section is really weak right now
% At a high level, our approach is to create a domain-specific language (DSL) which encompasses the set of transformations we want to support. Once we have defined a DSL, we can sample synthetic training data and use this to train a neural network to predict functions. This allows us to avoid the expensive data collection step of gathering spreadsheet data.

% There are two large assumptions implicit in this approach:

% First, that a neural model is capable of learning to recognize functions drawn from a language sufficiently rich to support a broad array of string transformations.

% Second, that the model learns a sufficiently deep understanding of function semantics, such that it can identify functions with the same semantics, even when they are applied to input data drawn from different distributions.

% We assess the validity of both these assumptions in Section \ref{sec:eval}

% % We use the FlashFill benchmark as our test set. The dataset consists of 245 real world examples of string transformation programs obtained from the Microsoft Excel team and online help forums. Example programs include repairing formatting for telephone numbers, or extracting specific address information from raw address strings. Each data point consists of a string transformation program, accompanied by at least 5 input-output examples for that program.


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{placeholder.png}
%     \caption{This is a placeholder image until we decide on a good example to go here. The actual example should have 5 output examples, and the rest autocompleted.\\ \\
%     An example from the FlashFill dataset. Here, the model must synthesize a program to extract names from email addresses them and properly format them. The solution our model finds is \texttt{Concat(ToLowercase(Select(Word, 1), ToLowerCase(Select(Word, 2)))}. }
%     \label{fig:ff_example}
% \end{figure}

% % We describe programs using the source code ordered linearization of the abstract syntax tree.

% \input{dsl}

% \subsection{Search Procedure}

% Our approach is further motivated by the difficulty of exact algorithmic manipulation, even for humans. It is often much easier for programmers to sketch out a solution than to write out the complete source code,

% We note that this second consideration is true for humans in addition to artificial neural networks. Programming is a highly iterative process - humans almost never write a program correctly on the first try - it is a process of trying new modifications, and then testing. Further, for many structured tasks, humans think of these tasks symbolically - while it is easy to move in function space using the abstraction of functions, actually implementing a function such as string manipulation by hand is very tedious.
